Distance Estimation for BLE-based Contact Tracing -- A Measurement Study

Mobile contact tracing apps are -- in principle -- a perfect aid to condemn the human-to-human spread of an infectious disease such as COVID-19 due to the wide use of smartphones worldwide. Yet, the unknown accuracy of contact estimation by wireless technologies hinders the broader use. We address this challenge by conducting a measurement study with a custom testbed to show the capabilities and limitations of Bluetooth Low Energy (BLE) in different scenarios. Distance estimation is based on interpreting the signal pathloss with a basic linear and a logarithmic model. Further, we compare our results with accurate ultra-wideband (UWB) distance measurements. While the results indicate that distance estimation by BLE is not accurate enough, a contact detector can detect contacts below 2.5 m with a true positive rate of 0.65 for the logarithmic and of 0.54 for the linear model. Further, the measurements reveal that multi-path signal propagation reduces the effect of body shielding and thus increases detection accuracy in indoor scenarios.

==> math.tex <==
% ------------------- math.tex ----------------------
% - abbreviations for commonly used math expressions

\newcommand\fc{f_\text{c}}
\newcommand\pift{2\pi f_\text{c} t}
\newcommand\piftdouble{4\pi f_\text{c} t}
\newcommand\real[1]{\mathrm{Re}\left\{#1\right\}}
\newcommand\imag[1]{\mathrm{Im}\left\{#1\right\}}
\newcommand\gT{g_\mathrm{T}(t)}
\newcommand\gR{g_\mathrm{R}(t)}
\newcommand\gTkT{g_\mathrm{T}(t-kT)}
\newcommand\AIm{A_{\mathrm{I},m}}
\newcommand\AQm{A_{\mathrm{Q},m}}
\newcommand\E[1]{\mathbb{E}\{#1\}}
\newcommand\Ex[1]{\mathbb{E}\{#1\}}
\newcommand\var[1]{\mathrm{var}(#1)}
\newcommand\ve{\mathbf}
\newcommand\m{\mathbf}
\newcommand\argmax[1]{\mathop{\text{argmax}}_{#1}}
\newcommand\argmin[1]{\mathop{\text{argmin}}_{#1}}
\newcommand\Pb{P_\text{b}}
\newcommand\Ps{P_\text{s}}
\newcommand\Pn{P_\text{n}}
\newcommand\Pc{P_\text{c}}
\newcommand\Pe{P_\text{e}}
\newcommand\Prob{\mathrm{Pr}}

\newcommand\efct{e}
\newcommand\mj{j}
\newcommand\jom{j\omega}
\newcommand\jomn{j\omega_0}
\newcommand\jomt{j\omega t}
\newcommand\jomnt{j\omega_0 t}
\newcommand\mjomnt{-j\omega_0 t}
\newcommand\ejOm{e^{j\Omega}}
\newcommand\ejomt{e^{j\omega t}}
\newcommand\ejomT{e^{j\omega T}}
\newcommand\emjomt{e^{-j\omega t}}
\newcommand\emjomtn{e^{-j\omega t_0}}
\newcommand\ejomnt{e^{j\omega_0 t}}
\newcommand\emjomnt{e^{-j\omega_0 t}}
\newcommand\omnt{\omega_0 t}
\newcommand\komnt{k \omega_0 t}
\newcommand\emst{e^{-st}}
\newcommand\si{\mathrm{si}}
\newcommand\dt{\mathrm{d}t}
\newcommand\di{\mathrm{d}}
\newcommand\dom{\mathrm{d}\omega}
\newcommand\dmin{d_\mathrm{min}}
\newcommand\SNR{\mathrm{SNR}}
\newcommand\GF{\mathrm{GF}}
\newcommand\dH{d_\mathrm{H}}
\newcommand\FT{\unitlength1mm\begin{picture}(9,2) \put (1,1)
{\circle{1.7}} \put(2,1){\line(1,0){5}} \put(8,1)
{\circle*{1.7}}\end{picture}}
\newcommand\IFT{\unitlength1mm\begin{picture}(10,2) \put (1,1)
{\circle*{1.7}} \put(2,1){\line(1,0){5}} \put(8,1)
{\circle{1.7}}\end{picture}}

% ----------------------------


==> texfig/DistErrorData/UWBerrorBoxPlotLoc1.tex <==
lq med uq lw uw
-0.03 0.09 0.25 -0.26 0.67
0.16 0.24 0.32 -0.08 0.55
0.08 0.22 0.32 -0.27 0.67
-0.07 0.06 0.30 -0.27 0.69
0.17 0.25 0.38 -0.03 0.60
-0.06 0.12 0.40 -0.26 0.74


==> texfig/DistErrorData/UWBerrorBoxPlotLoc2.tex <==
lq med uq lw uw
0.24 0.42 1.59 -0.93 3.49
0.20 0.40 1.34 -0.10 2.89
0.21 0.35 0.85 0.06 1.82
0.27 0.37 0.86 -0.03 1.75
0.20 0.39 0.67 -0.16 1.38
0.27 0.36 0.98 0.02 2.02


==> texfig/DistErrorData/UWBerrorBoxPlotLoc3.tex <==
lq med uq lw uw
0.62 0.79 1.09 -0.07 1.79
-0.46 -0.39 0.46 -1.79 1.58
-0.75 -0.48 0.23 -0.94 0.92
-0.84 -0.06 0.29 -1.15 1.81
-0.54 -0.10 0.31 -1.13 1.59
-1.04 -0.42 0.07 -1.46 1.72


==> texfig/DistErrorData/errorBoxPlot11_lin.tex <==
lq med uq lw uw
-1.00 0.89 3.35 -1.00 7.79
-1.10 0.38 2.35 -2.00 7.28
-1.60 -1.11 -0.13 -3.00 1.84
-2.97 -1.13 0.35 -4.00 4.29
-2.62 -1.63 -0.16 -5.00 3.29
-2.63 -0.66 0.32 -5.59 3.77


==> texfig/DistErrorData/errorBoxPlot11_logdist.tex <==
lq med uq lw uw
-0.71 0.60 3.15 -0.91 7.89
-0.91 -0.07 2.15 -1.71 5.35
-1.68 -1.40 -0.66 -2.58 0.43
-2.85 -1.66 0.15 -3.65 3.35
-3.07 -2.17 0.02 -4.25 3.89
-3.17 0.07 2.89 -5.10 9.75


==> texfig/DistErrorData/errorBoxPlot12_lin.tex <==
lq med uq lw uw
-1.00 -0.09 0.47 -1.00 2.16
-0.04 1.44 2.84 -2.00 4.53
-2.09 -0.69 0.72 -2.93 2.69
-1.12 -0.28 0.84 -2.25 2.25
-2.55 -0.86 0.26 -3.25 1.53
-2.14 -1.16 -0.59 -3.69 0.25


==> texfig/DistErrorData/errorBoxPlot12_logdist.tex <==
lq med uq lw uw
-0.27 0.11 0.37 -0.68 1.08
-0.35 0.84 2.79 -1.56 6.94
-1.89 -1.13 0.16 -2.19 2.89
-1.69 -0.84 0.79 -2.48 4.05
-3.02 -1.31 0.60 -3.48 3.94
-2.67 -1.21 -0.11 -4.63 2.05


==> texfig/DistErrorData/errorBoxPlot13_lin.tex <==
lq med uq lw uw
-0.73 -0.03 0.89 -1.00 3.21
-1.03 -0.34 0.59 -2.00 2.91
-1.11 0.05 1.21 -2.96 3.53
-0.25 0.44 1.60 -2.80 2.76
-0.79 -0.09 0.37 -1.71 1.53
-0.86 -0.40 0.24 -2.25 0.76


==> texfig/DistErrorData/errorBoxPlot13_logdist.tex <==
lq med uq lw uw
-0.15 0.12 0.61 -0.62 1.52
-0.88 -0.53 0.11 -1.50 1.31
-1.39 -0.48 0.96 -2.22 3.81
-0.69 0.34 2.81 -2.78 6.70
-1.04 0.20 1.23 -2.24 3.94
-0.31 0.81 2.74 -3.48 4.70


==> texfig/DistErrorData/errorBoxPlot21_lin.tex <==
lq med uq lw uw
-1.00 0.04 3.24 -1.00 6.43
-0.96 0.10 1.53 -2.00 5.08
-0.54 0.53 1.95 -3.00 4.43
-0.47 0.95 1.66 -3.67 3.43
-0.41 0.30 1.01 -2.19 2.79
-2.12 -1.41 -0.17 -4.96 2.14


==> texfig/DistErrorData/errorBoxPlot21_logdist.tex <==
lq med uq lw uw
-0.72 0.30 2.91 -0.95 8.22
-0.70 -0.12 1.06 -1.66 3.65
-0.88 0.06 2.00 -2.51 6.22
-0.94 1.00 2.38 -3.10 6.42
-0.58 0.65 2.21 -3.70 5.42
-2.54 -1.58 0.80 -4.85 5.77


==> texfig/DistErrorData/errorBoxPlot22_lin.tex <==
lq med uq lw uw
-1.00 -0.78 0.47 -1.00 2.65
-1.15 -0.22 0.40 -2.00 2.58
-0.60 0.49 1.90 -2.47 5.01
-0.97 0.27 1.52 -3.47 4.95
-1.04 -0.10 0.83 -3.53 3.32
-1.73 -0.48 0.77 -4.22 3.88


==> texfig/DistErrorData/errorBoxPlot22_logdist.tex <==
lq med uq lw uw
-0.38 -0.05 0.47 -0.74 1.54
-0.82 -0.36 0.04 -1.51 1.16
-0.96 -0.01 1.88 -1.94 5.42
-1.46 -0.07 2.07 -2.94 6.48
-1.48 -0.12 1.77 -3.53 5.48
-2.07 0.07 3.39 -4.36 10.21


==> texfig/DistErrorData/errorBoxPlot23_lin.tex <==
lq med uq lw uw
-1.00 -0.27 0.73 -1.00 2.93
-0.20 0.33 1.66 -1.80 4.32
-0.94 -0.14 0.66 -3.00 2.79
-0.07 0.99 1.53 -2.20 2.59
-0.54 0.26 0.79 -1.87 1.86
-1.01 -0.47 0.06 -2.07 0.59


==> texfig/DistErrorData/errorBoxPlot23_logdist.tex <==
lq med uq lw uw
-0.40 0.09 0.58 -0.75 1.64
-0.38 -0.03 1.22 -1.10 3.26
-1.22 -0.61 0.22 -2.19 2.26
-0.45 1.26 2.40 -2.54 5.48
-0.68 0.80 2.06 -2.36 5.46
-0.74 0.40 1.79 -2.45 3.48


==> texfig/DistErrorData/errorBoxPlot31_lin.tex <==
lq med uq lw uw
-1.00 -0.10 1.98 -1.00 6.15
-2.00 0.46 2.55 -2.00 6.20
-1.58 1.02 2.59 -3.00 5.20
-1.67 -0.50 1.07 -4.00 4.20
-2.54 -0.45 0.59 -5.00 4.76
-4.32 -2.76 -0.93 -6.00 3.24


==> texfig/DistErrorData/errorBoxPlot31_logdist.tex <==
lq med uq lw uw
-0.57 0.15 1.51 -0.98 4.49
-1.22 0.07 2.51 -1.71 7.85
-1.60 0.71 3.67 -2.93 11.56
-2.02 -0.95 1.49 -3.57 5.85
-2.93 -0.49 1.67 -4.57 6.98
-4.45 -3.22 -0.51 -5.22 3.85


==> texfig/DistErrorData/errorBoxPlot32_lin.tex <==
lq med uq lw uw
-1.00 -1.00 -0.04 -1.00 1.10
-0.47 1.24 2.95 -2.00 6.95
-1.47 0.81 3.67 -3.00 7.66
-1.90 -0.19 2.09 -4.00 7.80
-2.90 -0.62 1.67 -5.00 7.37
-3.33 -0.48 1.81 -6.00 5.80


==> texfig/DistErrorData/errorBoxPlot32_logdist.tex <==
lq med uq lw uw
-0.64 -0.37 0.31 -0.88 1.28
-0.42 0.74 2.76 -1.79 6.26
-1.42 0.29 5.26 -2.48 14.25
-2.10 -0.71 2.88 -3.56 7.94
-3.10 -1.04 3.26 -4.56 12.25
-3.72 -0.28 5.94 -5.37 18.92


==> texfig/DistErrorData/errorBoxPlot33_lin.tex <==
lq med uq lw uw
-0.58 -0.03 0.51 -1.00 1.79
-0.85 -0.49 0.24 -2.00 1.70
-1.49 -0.94 -0.03 -2.76 1.07
-0.48 0.07 0.61 -1.57 1.89
-1.12 -0.57 -0.21 -2.03 0.71
-1.48 -0.93 -0.39 -2.85 0.07


==> texfig/DistErrorData/errorBoxPlot33_logdist.tex <==
lq med uq lw uw
-0.11 0.11 0.39 -0.47 1.01
-0.80 -0.61 -0.13 -1.34 0.70
-1.61 -1.27 -0.49 -2.17 0.92
-0.86 -0.08 0.89 -1.99 3.09
-1.36 -0.46 0.27 -3.13 2.63
-1.28 -0.11 1.36 -3.30 2.85


==> texfig/DistErrorData/errorBoxPlotAll_lin.tex <==
lq med uq lw uw
-0.24 0.66 2.09 -1.00 5.14
-0.34 0.74 1.63 -2.00 3.96
-0.44 0.27 1.17 -2.77 2.96
-1.09 -0.19 0.53 -3.41 1.96
-1.73 -1.01 -0.29 -3.88 1.50
-2.55 -1.83 -1.29 -4.34 0.32


==> texfig/DistErrorData/errorBoxPlotAll_logdist.tex <==
lq med uq lw uw
0.04 0.47 1.54 -0.65 3.71
-0.53 0.22 1.12 -1.51 3.40
-0.93 -0.28 0.84 -2.26 3.20
-1.63 -0.66 0.40 -3.09 3.11
-2.28 -1.42 -0.29 -3.88 2.62
-3.08 -2.16 -1.29 -4.72 1.11


==> texfig/DistErrorData/errorBoxPlotLoc1_lin.tex <==
lq med uq lw uw
-1.00 0.29 2.98 -1.00 7.91
-1.16 0.18 1.98 -2.00 6.46
-1.71 -0.37 1.87 -3.00 5.46
-1.37 -0.02 1.32 -4.00 4.46
-2.37 -0.57 0.77 -5.00 4.81
-2.47 -1.13 -0.23 -5.61 2.91


==> texfig/DistErrorData/errorBoxPlotLoc1_logdist.tex <==
lq med uq lw uw
-0.64 0.34 2.60 -0.99 7.21
-0.87 -0.14 1.60 -1.87 4.96
-1.66 -0.81 2.01 -2.82 6.69
-1.81 -0.40 1.90 -3.58 7.42
-2.81 -0.76 1.96 -4.18 8.47
-2.95 -0.99 0.96 -5.31 5.42


==> texfig/DistErrorData/errorBoxPlotLoc2_lin.tex <==
lq med uq lw uw
-1.00 -1.00 1.39 -1.00 4.59
-2.00 0.39 2.39 -2.00 8.40
-1.01 0.59 2.59 -3.00 6.60
-1.61 -0.01 1.59 -4.00 6.00
-1.81 -0.61 0.99 -5.00 5.00
-2.41 -0.81 1.19 -6.00 4.40


==> texfig/DistErrorData/errorBoxPlotLoc2_logdist.tex <==
lq med uq lw uw
-0.49 -0.11 1.03 -0.92 3.06
-1.11 0.03 2.06 -1.81 6.10
-1.23 0.08 3.14 -2.49 9.27
-1.97 -0.47 2.14 -3.49 8.27
-2.32 -0.94 2.06 -4.23 7.27
-2.92 -0.65 4.69 -5.11 15.34


==> texfig/DistErrorData/errorBoxPlotLoc3_lin.tex <==
lq med uq lw uw
-0.89 -0.02 0.64 -1.00 2.82
-1.02 -0.36 0.51 -2.00 2.70
-1.14 -0.49 0.61 -3.00 2.79
-0.39 0.48 0.92 -2.14 2.67
-0.96 -0.30 0.35 -2.49 1.67
-1.52 -0.86 -0.43 -2.83 1.10


==> texfig/DistErrorData/errorBoxPlotLoc3_logdist.tex <==
lq med uq lw uw
-0.19 0.14 0.47 -0.65 1.45
-0.86 -0.53 0.07 -1.55 1.45
-1.40 -0.93 0.17 -2.31 2.27
-0.83 0.45 1.27 -2.95 4.06
-1.25 -0.16 1.25 -2.93 4.56
-1.55 -0.26 0.80 -3.93 3.56


==> texfig/DistErrorData/errorBoxPlotPos1_lin.tex <==
lq med uq lw uw
-1.00 -0.53 2.89 -1.00 6.66
-1.19 0.52 2.24 -2.00 6.00
-1.16 -0.13 0.55 -3.00 2.95
-1.48 -0.45 0.58 -4.00 3.32
-1.79 -1.11 -0.08 -3.50 2.32
-1.76 -0.74 -0.05 -4.16 2.34


==> texfig/DistErrorData/errorBoxPlotPos1_logdist.tex <==
lq med uq lw uw
-0.44 -0.06 2.45 -0.92 6.52
-0.93 0.05 1.93 -1.88 5.52
-1.42 -0.66 0.03 -2.77 2.10
-1.95 -0.97 0.48 -3.57 3.52
-2.34 -1.55 0.10 -3.61 3.57
-2.07 -0.20 1.52 -4.78 6.65


==> texfig/DistErrorData/errorBoxPlotPos2_lin.tex <==
lq med uq lw uw
-1.00 -1.00 2.03 -1.00 6.42
-2.00 0.35 2.04 -2.00 6.77
-0.98 0.37 2.39 -3.00 5.77
-0.97 1.05 2.40 -4.00 4.77
-1.30 0.39 1.74 -5.00 4.44
-2.30 -0.61 0.40 -6.00 3.44


==> texfig/DistErrorData/errorBoxPlotPos2_logdist.tex <==
lq med uq lw uw
-0.61 -0.29 1.56 -0.89 4.81
-1.11 0.03 1.64 -1.75 5.35
-1.20 -0.12 2.81 -2.44 8.73
-1.44 1.17 4.26 -3.44 12.67
-1.76 0.81 4.28 -4.20 11.67
-2.76 -0.19 2.26 -5.11 8.83


==> texfig/DistErrorData/errorBoxPlotPos3_lin.tex <==
lq med uq lw uw
-1.00 -1.00 0.94 -1.00 3.54
-2.00 -0.06 2.11 -2.00 8.17
-1.06 1.11 3.27 -3.00 8.04
-0.76 0.97 2.71 -4.00 6.61
-1.76 -0.03 2.14 -5.00 6.04
-3.20 -1.03 0.71 -6.00 4.61


==> texfig/DistErrorData/errorBoxPlotPos3_logdist.tex <==
lq med uq lw uw
-0.61 -0.18 0.75 -0.94 2.70
-1.29 -0.25 1.70 -1.84 5.84
-1.25 0.70 4.84 -2.75 13.60
-1.26 1.00 5.11 -3.55 12.60
-2.26 -0.00 5.58 -4.61 14.29
-3.64 -1.00 3.11 -5.47 10.60


==> texfig/DistErrorData/errorMetric11_lin.tex <==
0.57 3.19 0.49 0.68

==> texfig/DistErrorData/errorMetric11_logdist.tex <==
4.15 12.74 0.55 0.58

==> texfig/DistErrorData/errorMetric12_lin.tex <==
0.33 2.05 0.62 0.82

==> texfig/DistErrorData/errorMetric12_logdist.tex <==
1.09 3.47 0.70 0.68

==> texfig/DistErrorData/errorMetric13_lin.tex <==
0.07 1.28 0.80 0.87

==> texfig/DistErrorData/errorMetric13_logdist.tex <==
0.44 1.80 0.86 0.85

==> texfig/DistErrorData/errorMetric21_lin.tex <==
0.38 1.84 0.60 0.86

==> texfig/DistErrorData/errorMetric21_logdist.tex <==
0.69 2.39 0.66 0.81

==> texfig/DistErrorData/errorMetric22_lin.tex <==
0.10 1.68 0.81 0.86

==> texfig/DistErrorData/errorMetric22_logdist.tex <==
0.78 3.28 0.83 0.82

==> texfig/DistErrorData/errorMetric23_lin.tex <==
0.16 1.23 0.73 0.83

==> texfig/DistErrorData/errorMetric23_logdist.tex <==
0.45 1.68 0.80 0.79

==> texfig/DistErrorData/errorMetric31_lin.tex <==
0.62 3.24 0.57 0.72

==> texfig/DistErrorData/errorMetric31_logdist.tex <==
3.11 8.82 0.64 0.65

==> texfig/DistErrorData/errorMetric32_lin.tex <==
0.31 2.92 0.64 0.72

==> texfig/DistErrorData/errorMetric32_logdist.tex <==
2.28 7.98 0.70 0.66

==> texfig/DistErrorData/errorMetric33_lin.tex <==
0.00 0.95 0.85 0.90

==> texfig/DistErrorData/errorMetric33_logdist.tex <==
0.26 1.41 0.92 0.86

==> texfig/DistErrorData/errorMetricAll_lin.tex <==
0.39 2.42 0.61 0.78

==> texfig/DistErrorData/errorMetricAll_logdist.tex <==
1.49 4.53 0.65 0.74

==> texfig/DistErrorData/errorMetricLoc1_lin.tex <==
0.51 2.70 0.55 0.73

==> texfig/DistErrorData/errorMetricLoc1_logdist.tex <==
2.08 6.09 0.62 0.65

==> texfig/DistErrorData/errorMetricLoc2_lin.tex <==
0.27 2.44 0.66 0.75

==> texfig/DistErrorData/errorMetricLoc2_logdist.tex <==
1.64 5.70 0.70 0.71

==> texfig/DistErrorData/errorMetricLoc3_lin.tex <==
0.06 1.17 0.80 0.88

==> texfig/DistErrorData/errorMetricLoc3_logdist.tex <==
0.36 1.65 0.87 0.82

==> texfig/DistErrorData/errorMetricPos1_lin.tex <==
0.45 2.31 0.55 0.81

==> texfig/DistErrorData/errorMetricPos1_logdist.tex <==
1.60 4.80 0.61 0.73

==> texfig/DistErrorData/errorMetricPos2_lin.tex <==
0.28 2.22 0.64 0.79

==> texfig/DistErrorData/errorMetricPos2_logdist.tex <==
1.11 3.59 0.67 0.75

==> texfig/DistErrorData/errorMetricPos3_lin.tex <==
0.37 2.57 0.67 0.77

==> texfig/DistErrorData/errorMetricPos3_logdist.tex <==
1.62 5.04 0.72 0.72

==> texfig/DistErrorData/modelParam11_lin.tex <==
2.03 48.17 0.41

==> texfig/DistErrorData/modelParam11_logdist.tex <==
53.18 1.21 6.05

==> texfig/DistErrorData/modelParam12_lin.tex <==
3.56 42.77 0.60

==> texfig/DistErrorData/modelParam12_logdist.tex <==
51.62 2.21 6.87

==> texfig/DistErrorData/modelParam13_lin.tex <==
4.31 33.84 0.78

==> texfig/DistErrorData/modelParam13_logdist.tex <==
44.43 2.55 6.06

==> texfig/DistErrorData/modelParam21_lin.tex <==
2.81 45.08 0.56

==> texfig/DistErrorData/modelParam21_logdist.tex <==
51.52 1.88 6.49

==> texfig/DistErrorData/modelParam22_lin.tex <==
3.21 34.29 0.69

==> texfig/DistErrorData/modelParam22_logdist.tex <==
41.81 2.11 5.74

==> texfig/DistErrorData/modelParam23_lin.tex <==
3.76 38.25 0.78

==> texfig/DistErrorData/modelParam23_logdist.tex <==
47.17 2.34 4.87

==> texfig/DistErrorData/modelParam31_lin.tex <==
1.92 51.28 0.36

==> texfig/DistErrorData/modelParam31_logdist.tex <==
55.83 1.18 5.79

==> texfig/DistErrorData/modelParam32_lin.tex <==
1.75 44.32 0.45

==> texfig/DistErrorData/modelParam32_logdist.tex <==
48.29 1.25 5.77

==> texfig/DistErrorData/modelParam33_lin.tex <==
5.49 34.68 0.82

==> texfig/DistErrorData/modelParam33_logdist.tex <==
47.93 3.11 7.13

==> texfig/DistErrorData/modelParamAll_lin.tex <==
5.58 33.73 0.51

==> texfig/DistErrorData/modelParamAll_logdist.tex <==
47.51 3.36 8.48

==> texfig/DistErrorData/modelParamLoc1_lin.tex <==
2.92 43.62 0.51

==> texfig/DistErrorData/modelParamLoc1_logdist.tex <==
53.44 1.40 6.58

==> texfig/DistErrorData/modelParamLoc2_lin.tex <==
2.96 40.02 0.55

==> texfig/DistErrorData/modelParamLoc2_logdist.tex <==
45.88 1.66 7.34

==> texfig/DistErrorData/modelParamLoc3_lin.tex <==
2.72 43.86 0.49

==> texfig/DistErrorData/modelParamLoc3_logdist.tex <==
46.60 2.71 6.71

==> texfig/DistErrorData/modelParamPos1_lin.tex <==
2.92 43.62 0.51

==> texfig/DistErrorData/modelParamPos1_logdist.tex <==
50.80 1.77 6.58

==> texfig/DistErrorData/modelParamPos2_lin.tex <==
2.96 40.02 0.55

==> texfig/DistErrorData/modelParamPos2_logdist.tex <==
46.88 1.97 7.34

==> texfig/DistErrorData/modelParamPos3_lin.tex <==
2.72 43.86 0.49

==> texfig/DistErrorData/modelParamPos3_logdist.tex <==
50.27 1.76 6.71

==> texfig/tab_allvalues.tex <==
\begin{tabular}{ccc|ccc|c|cc}
Loc. & Pos. & Model & $\theta_1$ & $\theta_2$ & $\nu$ & RMSE & $r_p$ & $r_n$ \\ 
\hline
anec. & head & l-d & 53.2 & 1.21 & 6.05 & 3.89 & 0.61 & 0.49 \\ 
 &  & lin & 2.0 & 48.17 & 0.41 & 2.36 & 0.55 & 0.58 \\ 
 & trunk & l-d & 51.5 & 1.88 & 6.49 & 2.39 & 0.66 & 0.81 \\ 
 &  & lin & 2.8 & 45.08 & 0.56 & 1.84 & 0.60 & 0.86 \\ 
 & pelvis & l-d & 55.8 & 1.18 & 5.79 & 3.65 & 0.64 & 0.65 \\ 
 &  & lin & 1.9 & 51.28 & 0.36 & 2.40 & 0.64 & 0.65 \\ 
corr. & head & l-d & 51.6 & 2.21 & 6.87 & 1.86 & 0.74 & 0.63 \\ 
 &  & lin & 3.6 & 42.77 & 0.60 & 1.66 & 0.69 & 0.70 \\ 
 & trunk & l-d & 41.8 & 2.11 & 5.74 & 3.28 & 0.83 & 0.82 \\ 
 &  & lin & 3.2 & 34.29 & 0.69 & 1.68 & 0.81 & 0.86 \\ 
 & pelvis & l-d & 48.3 & 1.25 & 5.77 & 7.98 & 0.70 & 0.66 \\ 
 &  & lin & 1.8 & 44.32 & 0.45 & 2.92 & 0.64 & 0.72 \\ 
corn. & head & l-d & 44.4 & 2.55 & 6.06 & 1.65 & 0.86 & 0.85 \\ 
 &  & lin & 4.3 & 33.84 & 0.78 & 1.25 & 0.80 & 0.87 \\ 
 & trunk & l-d & 47.2 & 2.34 & 4.87 & 1.68 & 0.80 & 0.79 \\ 
 &  & lin & 3.8 & 38.25 & 0.78 & 1.23 & 0.73 & 0.83 \\ 
 & pelvis & l-d & 47.9 & 3.11 & 7.13 & 0.94 & 0.93 & 0.85 \\ 
 &  & lin & 5.5 & 34.68 & 0.82 & 0.90 & 0.89 & 0.87 \\ 
\hline
all & head & l-d & 50.8 & 1.77 & 6.58 & 2.56 & 0.64 & 0.66 \\ 
 &  & lin & 2.9 & 43.62 & 0.51 & 1.92 & 0.55 & 0.81 \\ 
 & trunk & l-d & 46.9 & 1.97 & 7.34 & 3.67 & 0.66 & 0.75 \\ 
 &  & lin & 3.0 & 40.02 & 0.55 & 2.23 & 0.64 & 0.80 \\ 
 & pelvis & l-d & 50.3 & 1.76 & 6.71 & 3.43 & 0.72 & 0.72 \\ 
 &  & lin & 2.7 & 43.86 & 0.49 & 2.26 & 0.67 & 0.77 \\ 
\hline
anec. & all & l-d & 53.4 & 1.40 & 6.58 & 3.36 & 0.61 & 0.65 \\ 
 &  & lin & 2.9 & 43.62 & 0.51 & 2.23 & 0.56 & 0.72 \\ 
corr. &  & l-d & 45.9 & 1.66 & 7.34 & 4.97 & 0.71 & 0.72 \\ 
 &  & lin & 3.0 & 40.02 & 0.55 & 2.32 & 0.67 & 0.76 \\ 
corn. &  & l-d & 46.6 & 2.71 & 6.71 & 1.30 & 0.91 & 0.79 \\ 
 &  & lin & 2.7 & 43.86 & 0.49 & 1.10 & 0.80 & 0.88 \\ 
\hline
all & all & l-d & 47.5 & 3.36 & 8.48 & 1.68 & 0.65 & 0.74 \\ 
 &  & lin & 5.6 & 33.73 & 0.51 & 1.57 & 0.54 & 0.86 \\ 
\hline
\end{tabular}
